High Throughput Low Delay Wireless Multicast via Multi-Channel Moving Window Codes

A fundamental challenge in wireless multicast has been how to simultaneously achieve high-throughput and low-delay for reliably serving a large number of users. In this paper, we show how to harness substantial throughput and delay gains by exploiting multi-channel resources. We develop a new scheme called Multi-Channel Moving Window Codes (MC-MWC) for multi-channel multi-session wireless multicast. The salient features of MC-MWC are three-fold. (i) High throughput: we show that MC-MWC achieves order-optimal throughput in the many-user many-channel asymptotic regime. Moreover, the number of channels required by a conventional channel-allocation based scheme is shown to be doubly-exponentially larger than that required by MC-MWC. (ii) Low delay: using large deviations theory, we show that the delay of MC-MWC decreases linearly with the number of channels, while the delay reduction of conventional schemes is no more than a finite constant. (iii) Low feedback overhead: the feedback overhead of MC-MWC is a constant that is independent of both the number of receivers in each session and the number of sessions in the network. Finally, our trace-driven simulation and numerical results validate the analytical results and show that the implementation complexity of MC-MWC is low.

==> sect31.tex <==
\section{MWNC with Infrequent Anonymous Feedback}\label{sec:IAF}

\begin{figure}[t]
\centering
  \includegraphics[width=3.5in]{figure/Batched_Feedback}
  %\vspace{-0.25cm}
  \caption{Illustration of MWNC with Infrequent Anonymous Feedback.}
  \vspace{-0.5cm}
  \label{fig:batched_feedback}
\end{figure}

We now propose an infrequent anonymous feedback policy that can
further reduce the feedback overhead to $1/B_{AF}$ of the original
MWNC-AF policy. In this policy, anonymous feedback is practiced once
for a frame of $B_{AF}$ packet transmissions, as shown in Figure
\ref{fig:batched_feedback}. If the transmitter cannot detect the
beacon signal, it will remove $B_{AF}$ packets from the encoder
buffer at the end of the frame. Otherwise, no packet will be
removed. If the uplink beacon-based feedback is reliable, we can
ensure that the removed packets are already seen at each receiver,
i.e., the multicast transmissions are reliable. We note that this
policy does not increase the decoding delay, because the decoding
delay is determined by the virtual decoder queue $Q_i[t]$ of each
receiver, and does not depend on the encoder queue $W[t]$. On the
other hand, this policy results in higher encoding and decoding
complexity, because the number of packets participating the encoding
procedure is increased.

If the uplink beacon-based feedback is not reliable, this policy
also provide an easy way to recover the throughput loss due to
feedback error. Specifically, we can postpone the removal time of
the packets by one frame, which provides an extra protection window
of size B_{AF}. In Figure ??, we plot ?? versus B_{AF} .....

Figure

So far, we have seen that the proposed anonymous feedback policy can
be easily generalized to reduce feedback overhead and cope with
feedback error. We further note that this policy can be used for FDD
systems with a minor change of the frame structure: the feedback
time interval can be replaced by a specific feedback frequency
channel. The transmitter broadcast $A[t]$ and $Z[t]$ to the
receivers at the beginning of each frame, and the receivers keep
sending feedback beacon signals during the frame.

